On Stein's Identity and Near-Optimal Estimation in High-dimensional Index Models

We consider estimating the parametric components of semi-parametric multiple index models in a high-dimensional and non-Gaussian setting. Such models form a rich class of non-linear models with applications to signal processing, machine learning and statistics. Our estimators leverage the score function based first and second-order Stein's identities and do not require the covariates to satisfy Gaussian or elliptical symmetry assumptions common in the literature. Moreover, to handle score functions and responses that are heavy-tailed, our estimators are constructed via carefully thresholding their empirical counterparts. We show that our estimator achieves near-optimal statistical rate of convergence in several settings. We supplement our theoretical results via simulation experiments that confirm the theory.

==> method.tex <==
%!TEX root = main.tex

%\section{Estimation via Score Functions}\label{sec:method}


%We now ascribe a version of Stein's Lemma that is applicable for non-Gaussian random variables. Recall from the motivating example for the Gaussian case in \S\ref{sec:intro} that while utilizing the Stein's Lemma for SIM estimation, assumptions on the function in Stein?s Lemma translate directly to those on the link function in SIM.  We now introduce a version of Stein's Lemma that applies to non-Gaussian random variables and for continuously differentiable functions from~\cite{stein2004use}. A more general version of the Stein's Lemma that applies to a class of regular functions is available in~\cite{stein2004use}. We assume continuously differentiable functions in the Stein's Lemma below as they cover a wide range of practical SIM such as generalized linear models and single-layer neural networks.  

%class of functions that is required in order to state Stein's Lemma. Following~\cite{stein2004use} a function is called regular, if it is finite on its domain (interior and its boundary),  both right and left limit exists on all points on its interior and the limits from the interior exists on the boundary of the domain. Based on the above definition, we have the  following  version of Stein's Lemma.
%\begin{lemma}[Non-Gaussian Stein's Lemma~\cite{stein2004use}]\label{lemma:stein_identity2}
%Let $g\colon \RR^{d }  \rightarrow \RR$ be continuously differentiable function and $X \in \RR^d$ be a random vector with density $p \colon \RR^{d} \rightarrow \RR$, which is also continuously differentiable. Under the assumption that the expectations $\EE    [ g(X) \cdot S(X)   ]$ and $ \EE   [ \nabla g(X)   ]$ are both well-defined, we have the following generalized Stein's identity  
%\#\label{eq:stein_identity2}
%\EE    [ g(X) \cdot S(X)   ] =  -   \int_{\RR^d} g(x) \cdot \nabla p(x) \ud x &= \int_{\RR^d} \nabla g(x) \cdot p(x) \ud x = \EE   [ \nabla g(X)   ] .
%\#
%\end{lemma}

%\#\label{eq:stein_identity2} == REPLACE ABOVE WITH THIS AFTER ICML VERSION
%\EE    [ g(X) \cdot S_{jk} (X)   ] = -  \int_{\RR^d} g(x) \cdot \nabla p(x) \ud x = \int_{\RR^d} \nabla g(x) \cdot p(x) \ud x = \EE   [ \nabla g(X)   ].
%\#

Recall that in  the two single index models introduced in \S \ref{sec:model}, $X$ in \eqref{eq:sim_model} has i.i.d. entries with density $p_0$.  To unify both the vector and matrix settings,  in the low-rank SIM, we identify   $X$ with $\vec(X) \in  \RR^{d }$ where $d = d_1\cdot d_2$. In this case, $X$ has density  $p = p_0^{\otimes d}$ and the corresponding  score function  $S \colon \RR^{d } \rightarrow \RR  ^{d  }$ is given by
\#\label{eq:def_score}
S (x) = - \nabla \log p(x)=  - \nabla p (x) / p  (x)  =  s_0\circ(x ),
\#  
where  the univariate function $s_0 = p_0'  /  p_{0} $ is applied to each entry of $x$.
Thus   $S(X) $ has i.i.d. entries. In addition, by Lemma \ref{lemma:stein_identity2},  we have $\EE [S(X) ] = 0$ by setting $g$ to be a constant function in \eqref{eq:stein_identity2}. Moreover, in the context of SIMs specified in \eqref{eq:sim_model}, we have 
\$
\EE [ Y \cdot   S(X)    ] = \EE \bigl [ f( \la X , \beta^*\ra) \cdot S(X) \bigr] = \EE   [ f' ( \la X ,  \beta ^* \ra ) ] \cdot  \beta ^*,
\$
as long as the density and the link function satisfy the conditions stated in Lemma~\ref{lemma:stein_identity2}. This implies that optimization problem 
\#\label{eq:opt_population}
\minimize _{\beta \in \RR^d }  \bigl\{ \la \beta , \beta \ra - 2 \EE [ Y \cdot   \la S(X) , \beta \ra    ]  \bigr\} 
\#
has solution $\beta =  \mu \cdot \beta ^* $, where $ \mu =\EE   [ f' ( \la X ,  \beta ^* \ra ) ] $. Hence the above program could be used to obtain the unknown $\beta^*$ as long as $\mu \neq 0$. Before we proceed to describe the sample version of the above program, we make the following brief remark. The requirement $\mu \neq 0$ rules out in particular the use of our approach for non-Gaussian phase retrieval (where $f(u) = u^2$) as in that case we have $\mu =0$ when $X$ is centered. But we emphasize that the same holds true in the Gaussian and elliptical setting as well, as noted in~\cite{plan2015generalized} and \cite{goldstein2016structured}. Their methods also fail  to recover the true $\beta^*$ when the SIM model corresponds to phase retrieval. We refer the reader to \S\ref{sec:conclusion} for a discussion on overcoming this limitation.

Finally, we use a sample version of the above program as an estimator for the unknown $\beta^*$. In order to deal with the high-dimensional setting, we consider a regularized version of the above formulation. More specifically, we use the $\ell_1$-norm and nuclear norm regularization   in the vector and matrix settings respectively. However, a major difficulty in the sample setting for this procedure is that $\EE[ Y \cdot S(X) ]$ and its empirical counterpart may not be close enough due to  a lack of concentration. Recall our discussion from \S\ref{sec:challenges} that even if the random variable $X$ is light-tailed, its score-function $S(x)$ might be arbitrarily heavy-tailed.  Furthermore,   bounded-fourth moment assumption on the noise, $Y$ too can be heavy-tailed.  Thus the naive method of using the sample version of  \eqref{eq:opt_population} to estimate $\beta^*$ leads to sub-optimal statistical rates of convergence.
%{\color{red} Revise this: For example, when $\beta^*$ is assumed to be sparse, we estimate the it by solving the empirical version of \eqref{eq:opt_population} with $\ell_1$-regularization. Whereas when $\beta^*$ is   low-rank, we use the nuclear norm penalty to enforce the low-rank structure. }
%Furthermore, under the distributional assumption on the score and the noise~\textcolor{red}{what is the assumption on $\epsilon$? {\color{blue} bounded 4-th moments} Need to clarify this part here} of $Y$ too is heavy-tailed.  Thus the naive method may incur large estimation error. 

To improve concentration and obtain optimal rates of convergence, we replace $Y \cdot S(X)$ with a transformed random variable $\cT(Y, X)$, which will be defined precisely in  \S \ref{sec:theory} for the sparse and low-rank cases. In particular, $\cT(Y, X)$ is a carefully truncated version of $Y \cdot S(X)$, introduced and analyzed in \cite{catoni2012challenging, fan2016robust} for related problems, that enables us to obtain well-concentrated estimators. Thus our final estimator $\hat \beta$ is defined as the solution to  the following regularized  optimization  problem
\#\label{eq:estimator}
\minimize _{ \beta \in \RR^d} ~L(\beta)   + \lambda \cdot R(\beta),~~L(\beta) = \la \beta , \beta \ra   - \frac{2}{n} \sum_{i=1}^n  \la \cT(Y_i, X_i) ,  \beta\bigr \ra, 
\#
where $\lambda>0$ is the regularization parameter which will be specified later and $R(\cdot)$ is the $\ell_1$-norm in the vector case and the nuclear norm in the matrix case. 


==> tensor.tex <==
%!TEX root = ../main.v1.tex

\subsection{Low-rank Tensor Single Index Model}

Before we lay out the low-rank tensor single index model, we first introduce additional notation for tensors. Throughout this paper, for any  fourth-order tensor $ Z \in \RR^{d_1 \times d_2 \times d_3 \times d_4 }$, we denote its $(j_1,j_2, j_3, j_4)$-th entry by $Z (j_1, j_2, j_3, j_4)$. For ease of presentation, we assume $d_{\ell} = d $ for all $\ell \in [4]$ and denote $Z \in \RR^{d ^\otimes 4}$, though our results holds for general $(d_1, d_2, d_3, d_4)$. Similar to the matrix case, we define $\vec(Z) \in \RR^{d^4}$ as the vectorization of the tensor  $Z$.  For two tensors $W,  Z \in \RR^{d^\otimes 4} $, we define their inner inner product  as
\#\label{eq:tensor_inner}
 \la Z, W \ra = \vec(Z)^\top \vec(W) = \sum_{j_1 , j_2, j_3, j_4 \in [d]} Z(j_1, j_2, j_3, j_4) \cdot W(j_1, j_2, j_3, j_4)
\#
The tensor Frobenius norm of    is denoted by $\| \cdot  \|_{\fro} $.
In addition,  we denote by $ \mat \colon \RR^{d ^ \otimes 4  }  \rightarrow \RR^{d^2 \times d^2 }$ the  operation of tensor unfolding, which maps a fourth-order tensor to a matrix. More specifically, the entries of $\mat(Z)$ are specified by
$ [ \mat (Z)]_{k_1, k_2} = Z ( j_1, j_2, j_3, j_4)
$,
$ \mat (Z+ W)  = \mat (Z) + \mat (W)$ for any two tensors $Z$ and $W$.
Based on tensor unfolding, we  define the matricized tensor nuclear norm as the matrix nuclear norm of the unfolded tensor, that is,
$
\| Z \|_{\tnuc} = \| \mat(Z)   \|_{\nuc}.
$
Thus the dual norm of $\| \cdot \|_{\tnuc}$ is given by
$
\| Z \|_{\toper} =  \| \mat (Z)  \|_{\oper}.
$
Furthermore, we denote by $ u  \otimes v     \otimes s \otimes t \in\mathbb{R}^{d ^ \otimes 4 }  $ a rank-one tensor. We say the tensor $Z$  is rank-$r$, denoted by $\rank(Z) = r$,  if it can be written as a summation of $r$ rank-one tensors, i.e.,
$
Z = \sum_{j= 1}^r \lambda_j u_j \otimes v_j \otimes s_j \otimes  t_j,
$
where $\lambda_j \in \RR$, $u_j$, $v_j$, $s_j$,  and $t_j$ are unit vectors.

The operator norm of a tensor is defined as
$$
\|Z \|_{\oper} =   \sup \left \{ \langle Z, u  \otimes v \otimes w  \rangle\colon u , v, s, t \in \RR^d,    \| u\|_2 = \| v \|_2 = \| s\|_2  =  \| t \|_2 = 1 \right \}.
$$
In addition, the tensor nuclear norm is defined as the dual of the tensor operator norm  ~\citep{yuan2014tensor}
\#\label{eq:tensor_nuc}
\|Z \|_{\nuc} = \sup\left \{ \langle  Z, W\rangle \colon \| W \|_{\oper} \leq 1 \right \}.
\#

Based on tensor unfolding operation, we define the matricized tensor nuclear norm as the matrix nuclear norm of the unfolded tensor, that is,
$
\| Z \|_{\tnuc} = \| \mat(Z)   \|_{\nuc}.
$
Thus the dual norm of $\| \cdot \|_{\tnuc}$ is given by
$
\| Z \|_{\toper} =  \| \mat (Z)  \|_{\oper}.
$

The operator norm of a tensor is defined as
$$
\|Z \|_{\oper} =   \sup \left \{ \langle Z, u  \otimes v \otimes w  \rangle\colon u , v, s, t \in \RR^d,    \| u\|_2 = \| v \|_2 = \| s\|_2  =  \| t \|_2 = 1 \right \}.
$$
In addition, the tensor nuclear norm is defined as the dual of the tensor operator norm  ~\citep{yuan2014tensor}
\#\label{eq:tensor_nuc}
\|Z \|_{\nuc} = \sup\left \{ \langle  Z, W\rangle \colon \| W \|_{\oper} \leq 1 \right \}.
\#

\subsection{Formulation}



{\bf \noindent Tensor single index model:} Let $X , \beta^* \in \RR^{d ^{\otimes 4}}
 $ be fourth-order tensors.  We assume that $\beta^*$ is a  rank $r^*$ tensor and the response variable $Y$ is defined by \eqref{eq:sim_model}, where the inner product is  defined in \eqref{eq:tensor_inner}. In addition,  we also assume $ \| \beta \|_{\fro}  = 1$.

It is worth noting that since   $\beta^*$ is low-rank, the unfolded tensor,  $\mat(\beta^*)$ is a low-rank matrix in $\RR^{d^2 \times d^2}$. Thus the tensor SIM can be learned by applying the estimation method for low-rank SIM. See   \S \ref{sec:theory} for details.


\subsection{Tensor Single Index Model}
Now we present the main result for the tensor SIM. Since the true parameter $\beta ^*$ is low-rank, we choose the regularization term $R(\beta)$ in \eqref{eq:estimator} to promote low-rankness in the solution. Similar to the matrix case, a tempting choice is the tensor nuclear norm defined in \eqref{eq:tensor_nuc}. However, we remark that such a norm is NP-hard to compute in the worst-case even though it has superior statistical properties.


Therefore,  to obtain an estimator which is computationally efficient, we utilize the   matricized nuclear norm  $\| \cdot \| _{\tnuc} $ for regularization. Since  tensor unfolding is a linear operation, $\mat (\beta ^*)$ is a rank-$r^*$ matrix in $\RR^{d^2 \times d^2}$. Thus


Recall that in the tensor setting, $S(X) \in \RR^{d ^ \otimes 4}$ has i.i.d. entries. Similar to the vector and matrix cases, we need to construct the mapping $\cT$ such that $n^{-1} \sum_{i=1}^n \cT(Y_i, X_i)$ is close to $\EE [ Y S(X) ]$ in the dual norm of $\| \cdot \|_{\tnuc}$. As shown in \S \ref{sec:model}, the dual norm of $\| \cdot \|_{\tnuc} $ is the  operator norm of the unfolded tensor.
Thus similar to  \S \ref{sec:lowrank}, we apply the truncation to $ Y \cdot \mat [ S(X)]$  to construct $\cT(Y, X)$ which is well-behaved under norm $\| \cdot \|_{\tnuc}$.   



 %Apart from the above norms, one could also enforce low Tucker-rank structures on the tensors. Let $\textsc{m}_{j}(\cdot): \mathbb{R}^{d_1 \times d_2 \times \ldots \times d_p} \mapsto \mathbb{R}^{d_j \times (d_1d_2\cdots d_{j-1}d_{j+1}\cdots d_p) }$ be the mode-$j$ matricization of a given tensor. Then the matricized tensor nuclear-norm is defined as:
\begin{align*}
\|\mathbf{X}\|_{**} = \frac{1}{p}\sum_{j=1}^p \| \textsc{m}_j(\mathbf{X})\|_*
\end{align*}
Although $\|\mathbf{X}\|_{**} $ is easy to compute, it has been noted to have inferior statistical properties compared to the regular tensor nuclear norm $\|\mathbf{X}\|_{*}$ \cite{yuan2014tensor}. {\color{red} Not low-rank?} In this paper, we assume that parameter tensor lies in a radius-r ball with respect to any of the above tensor norms, i.e., $\mathbf{W} \in \mathcal{K} =  \{ \mathbf{V}: \|V\| \leq r\}$, where $\|\cdot\|$ is one of the above tensor norms depending on the application.

